Domination Mappings into the Hamming Ball: Existence, Constructions, and Algorithms

The Hamming ball of radius $w$ in $\{0,1\}^n$ is the set ${\cal B}(n,w)$ of all binary words of length $n$ and Hamming weight at most $w$. We consider injective mappings $\varphi: \{0,1\}^m \to {\cal B}(n,w)$ with the following domination property: every position $j \in [n]$ is dominated by some position $i \in [m]$, in the sense that "switching off" position $i$ in $x \in \{0,1\}^m$ necessarily switches off position $j$ in its image $\varphi(x)$. This property may be described more precisely in terms of a bipartite \emph{domination graph} $G = ([m] \cup [n], E)$ with no isolated vertices, for all $(i,j) \in E$ and all $x \in \{0,1\}^m$, we require that $x_i = 0$ implies $y_j = 0$, where $y = \varphi(x)$. Although such domination mappings recently found applications in the context of coding for high-performance interconnects, to the best of our knowledge, they were not previously studied. In this paper, we begin with simple necessary conditions for the existence of an $(m,n,w)$-domination mapping $\varphi: \{0,1\}^m \to {\cal B}(n,w)$. We then provide several explicit constructions of such mappings, which show that the necessary conditions are also sufficient when $w=1$, when $w=2$ and $m$ is odd, or when $m \le 3w$. One of our main results herein is a proof that the trivial necessary condition $|{\cal B}(n,w)| \ge 2^m$ for the existence of an injection is, in fact, sufficient for the existence of an $(m,n,w)$-domination mapping whenever $m$ is sufficiently large. We also present a polynomial-time algorithm that, given any $m$, $n$, and $w$, determines whether an $(m,n,w)$-domination mapping exists for a domination graph with an equitable degree distribution.

==> section7.tex <==
%\begin{comment}
%\vspace{1cm}
%
%There are many questions which remained unsolved and they are subject for future research.
%On some of these problem we will present some directions for their solution.
%\begin{enumerate}
%\item A construction for $w=3$, $w=4$, and for higher values of $w$.
%In contrary to the construction for $w=2$ we believe it would be extremely
%difficult to have a construction which attains $n_\text{min} (m,w)$.
%But, for such a construction we would like to mimic the construction for $w=2$.
%If for $w=2$ we used a recursion from $2\ell-1$ to $2\ell+1$, then for $w=3$ we
%would like to use a recursion from $2\ell -\epsilon$ to $2\ell+3 -\epsilon$.
%To form a domination mapping $\varphi$ we should construct two descendant arrays $A(\varphi)$
%and $B(\varphi)$. For $A(\varphi)$ we consider a representation of $A_1 A_2$, where $A_1$ has
%three columns and $A_2$ has $2\ell -\epsilon$ columns. $B(\varphi)$ is represented by
%$B_1 B_2$. We should distinguish between eight cases depending on the value of the three columns in $A_1$.
%
%\item We would like to see an existence proof of $(m,n,w)$-domination mapping for more set
%of parameters. It can be along the lines presented in this paper, but with more simplicity.
%A completely new idea for the proof is very welcomed.
%
%\item We would like to see more bounds related to the structure of the coordinates sequence.
%\end{enumerate}
%
%????????????????????
%\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

